Renewal structure of the Tree Builder Random Walk

In this paper, we study a class of random walks that build their own tree. At each step, the walker attaches a random number of leaves to its current position. The model can be seen as a subclass of the Random Walk in Changing Environments (RWCE) introduced by G. Amir, I. Benjamini, O. Gurel-Gurevich and G. Kozma. We develop a renewal framework for the process analogous to that established by A-S. Sznitman and M. Zerner in the context of RWRE. This provides a more robust foundation for analyzing the model. As a result of our renewal framework, we estabilish several limit theorems for the walker's distance, which include the Strong Law of Large Numbers (SLLN), the Law of the Iterated Logarithm (LIL), and the Invariance Principle, under an i.i.d. hypothesis for the walker's leaf-adding mechanism. Further, we show that the limit speed defined by the SLLN is a continuous function over the space of probability distributions on $\mathbb{N}$.

==> grand_coupling.tex <==
\section{The Grand Coupling}
Our next goal is to prove Theorem \ref{t:1}, which states that the speed $v(p)$ of the Bernoulli instance of the TBRW is continuous on $p$. We will leverage the formula for $v(p)$ provided by Theorem \ref{t:lln}. However, we will need a way to compare TBRW with different parameters $p$'s. In order to do this, we will create a grand coupling that allows us to see all the Bernoulli instances of the TBRW walking on the same tree.

More precisely, we will construct a Markov Chain $\dproc{(\mathcal{T}_n, \mathcal{X}_n)}{n}$ from which we can to recover the trajectory and tree of a TBRW generated by a sequence $\xi$ with $\xi_n = {\rm Ber}(p)$ for any $p \in [0,1]$. In this context, $\mathcal{T}_n$ will be a tree from which we can to extract $T_n^{(p)}$ which denotes the tree generated by a Bernoulli instance of the TBRW with parameter $p$ after $n$ steps. Whereas $\mathcal{X}_n$ will be a vector that will store the position of different instances of the TBRW and from which we obtain $X^{(p)}_n$.

Before we start the construction, let us describe in a high-level how the model works and some of the terminology employed in its definition. In the process $\dproc{(\mathcal{T}_n, \mathcal{X}_n)}{n}$ we have a list of balls moving over the vertices of the tree $\mathcal{T}$'s. The balls have labels that are subintervals of the interval $[0,1]$. A ball labeled $[a,b]$ that jumps to a vertex $v$ represents a {\it swarm} of walkers with parameters lying in $[a,b]$ jumping to $v$. In other words, we are moving blocks of walkers all at once. The vertices of $\mathcal{T}$ are labeled too. Their labels are union of subintervals of the interval $[0,1]$. The interpretation is that some vertices are visible only to TBRW's whose parameter belongs to some of the subintervals in the vertex's label. For instance, a vertex whose label is $[0,1/4] \cup[2/3]$ is visible only by walkers whose parameter is contained belongs to $[0,1/4]$ or~$[2/3,1]$. Moreover, there is a bijection between the vertices of $\mathcal{T}_n$ and the entries of $\mathcal{X}_n$ in a way that the $i$th entry of $\mathcal{X}_n$ stores what balls are in the $i$th vertex of $\mathcal{T}_n$. Since the vertices and balls have labels that are subintervals, we will say that a fixed $p$ belongs to a ball meaning that $p$ is in the subinterval which is the label of that ball.

We will construct the process $\dproc{(\mathcal{T}_n, \mathcal{X}_n)}{n}$ inductively. Recall that we want to couple all the Bernoulli instances starting from the same initial state $(T,x)$. We let $\mathcal{T}_0$ be $T$, which is a finite rooted tree. We also enumerate all of its vertices. Also, we label each vertex of $\mathcal{T}_0$ as the interval $[0,1]$. We also set $\mathcal{X}_0$ to be a list of length $|T|$. All of its entries are zeros, expect from the $x$-th one, which holds a ball whose label is $[0,1]$. See Figure \ref{fig:supert0} below.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.65\linewidth]{super_tree_t0.png}
    \caption{The tree $\mathcal{T}_0$ with its labeled vertices. And $\mathcal{X}_0$ storing the information that there is one ball labeled $[0,1]$ on $v_3$.}
    \label{fig:supert0}
\end{figure}

We obtain then $(\mathcal{T}_1, \mathcal{X}_1)$ from $(\mathcal{T}_0, \mathcal{X}_0)$ as follows. We sample independently of all the past a real number from a uniform random variable $U_1$ over $[0,1]$. Then, we add a new vertex $v$ to $x$ in $\mathcal{T}_0$ with label $[U_1,1]$. This is $\mathcal{T}_1$.

To obtain $\mathcal{X}_1$, firstly we delete the ball on vertex $x$ whose label was $[0,1]$ and add two new balls to vertex $x$: one with label $[0,U_1]$ and another one with label $[U_1,1]$. Notice that the new vertex added to $\mathcal{T}_0$ at $x$ is only visible by the ball with label~$[U_1,1]$. Then, we move each ball independently. The ball whose label is $[0,U_1]$ jumps to a randomly chosen vertex of $\mathcal{T}_1$ whose label contains (in the sense of sets) its label $[0,U_1]$. In this case, the ball $[0,U_1]$ can only jump to an old vertex of $\mathcal{T}_0$ because all of them were labeled $[0,1]$. We next move the ball labeled $[U_1,1]$. This ball also jumps to a uniformly chosen vertex among all the vertices whose label contains the interval $[U_1,1]$. Notice that this particular ball can jump to the new vertex.

Secondly, we enlarge $\mathcal{X}_0$ by one because we have added a single new vertex. Then $\mathcal{X}_1$ stores the position of the two new balls. For instance, if the ball labeled $[0,U_1]$ jumped to vertex $j$, then the $j$-th entry of $\mathcal{X}_1$ stores the interval $[0,U_1]$. If both balls jumped to a vertex $i$, then the $i$-th entry of $\mathcal{X}_1$ stores the list $\{[0,U_1], [U_1,1]\}$. Figure \ref{fig:supert1} below illustrates the two possible ways to obtain $(\mathcal{T}_1, \mathcal{X}_1)$. In the first one, we have two balls on different vertices. Whereas in the second one, the two balls moved together.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{super_tree_t1.png}
    \caption{Illustration of the two possible states of $(\mathcal{T}_1, \mathcal{X}_1)$}
    \label{fig:supert1}
\end{figure}

We will detail how to generate $(\mathcal{T}_2,\mathcal{X}_2)$ since it encodes the subtleties of the general case. We begin generating $\mathcal{T}_2$. As before, we first sample a real number from $U_2$, which is independent of the past. Following the vertices order, we add a new vertex to each vertex of $\mathcal{T}_1$ that is occupied according to $\mathcal{X}_1$. Now we need to know how to label each of these new vertices. Suppose a vertex $v_i$ is occupied by a set of balls whose labels are disjoint subintervals, let's say, $[a_1,b_1], [a_2,b_2]$. We then add a vertex to $v_i$ labeled as $[U_2,1]\cap ([a_1,b_1]\cup[a_2,b_2])$. Following this procedure for each occupied vertex gives us $\mathcal{T}_2$.

The vector $\mathcal{X}_2$ is obtained as follows: firstly we enlarge $\mathcal{X}_1$ to accommodate the new vertices added during the step of construction of $\mathcal{T}_2$. Secondly, observe that the labels of the balls form a partition of the interval $[0,1]$. Thus, almost surely, $U_2$ belongs to only one interval, let's say $[a_1,b_1]$, which is the label of a given ball. We then remove this ball and replace it by two new balls with labels $[a_1,U_2]$ and $[U_2,b_2]$. Finally, we let each ball jump to a neighbor chosen uniformly among all those neighbors whose label contains the ball's label. Figure \ref{fig:supertreet2} below illustrates a transition from step $1$ to $2$ in which $U_2 < U_1$.
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{super_treet2.png}
    \caption{Obtaining $(\mathcal{T}_2,\mathcal{X}_2)$ from $(\mathcal{T}_1,\mathcal{X}_1)$. In this case, $U_2 < U_1$.}
    \label{fig:supertreet2}
\end{figure}

Suppose we have successfully defined the first $k$ steps of $\{(\mathcal{T}_j, \mathcal{X}_j)\}_{j=0}^k$. The $(k+1)$th step is obtained exactly as $(\mathcal{T}_2, \mathcal{X}_2)$. In a nutshell, we add a new vertex to each occupied vertex of $\mathcal{T}_k$. Each of these vertices are occupied by a list of balls whose labels are disjoint subintervals of $[0,1]$. If a vertex $v$ is occupied by balls whose labels are $\{[a_{i_1}, b_{i_1}], \dots, [a_{i_l}, b_{i_l}]\}$, the new vertex added to $v$ is labeled as $[U_{k+1},1] \cap ([a_{i_1}, b_{i_1}] \cup \dots \cup [a_{i_l}, b_{i_l}])$. This gives us $\mathcal{T}_{k+1}$.

The vector $\mathcal{X}_{k+1}$ is obtained by firstly increasing the length of $\mathcal{X}_{k}$ accordingly since we added new vertices. The ball whose label is $[a_i,b_i]$ and contains $U_{k+1}$ is removed and replaced by two balls whose labels are $[a_i,U_{k+1}]$ and $[U_{k+1},b_i]$. Secondly, we let all the balls, including the two new ones, jump independently of each other and respecting the restriction that only vertices whose labels contain their label are available.

This construction gives us a probability space $\left(\Omega, \mathcal{F}, \cPl_{T,x} \right)$ , where $\Omega$ is the set of sequences of pairs of the type $(\mathcal{T}, \mathcal{X})$, where $\mathcal{T}$ is a finite rooted tree whose vertices are labeled as subintervals of $[0,1]$ and $\mathcal{X}$ is a vector of length $\mathcal{T}$ whose entries are either $0$ or lists of subintervals of $[0,1]$. And $\cPl_{T,x}$ is the law of the above defined process $\{(\mathcal{T}_n, \mathcal{X}_n)\}_{n}$.

The next step is to show that $\left(\Omega, \mathcal{F}, \cPl_{T,x} \right)$ provides a coupling between all Bernoulli instances of the TBRW for any $p\in [0,1]$. That is, we can see all TBRW with an i.i.d. Bernoulli sequence walking on the same tree. We will also have estimates on the probability that two different walkers walk together for a fixed number of steps.
\begin{theorem}[The Grand Coupling]\label{t:gc} For any finite initial state $(T,x)$, let $\left(\Omega, \mathcal{F}, \cPl_{T,x} \right)$ be the probability space  where $\cPl_{T,x}$ is the law of the process $\{(\mathcal{T}_j, \mathcal{X}_j)\}_{j}$. Then the following statements are true
\begin{enumerate}[label = (\alph*)]
    \item For each $p \in [0,1]$, there exists a process $\left \lbrace\left( T_n^{(p)}, X_n^{(p)}\right)\right \rbrace_{n \in \mathbb{N}}$ in $\left(\Omega, \mathcal{F}, \cPl_{T,x} \right)$ distributed as a Bernoulli instance of the TBRW with parameter $p$ and starting from $(T,x)$;

    \item for any $n \in \mathbb{N}$, 
    \begin{equation*}
        \cPl_{T,x} \left( \left \lbrace\left( T_k^{(p)}, X_k^{(p)}\right)\right \rbrace_{k=0}^n = \left \lbrace\left( T_k^{(q)}, X_k^{(q)}\right)\right \rbrace_{k=0}^n  \right) \ge (1-|p-q|)^n;
    \end{equation*}

    \item if $\ver{n}{p}$ denotes the number of vertices added by the walker $X^{(p)}$ after $n$ steps, then
    \begin{equation*}
        \ver{n}{p} \le \ver{n}{q}, \; \cPl_{T,x}\text{-a.s.},
    \end{equation*}
    for any $0 \le p \le q \le 1$.
\end{enumerate}

\end{theorem}

\begin{proof}  
We begin by part (a) of the theorem.\\

\noindent \underline{\it Part (a).} For each $p$, we let $T_n^{(p)}$ be the graph obtained from $\mathcal{T}_n$ by keeping only its vertices whose label contains $p$. We also let $X_n^{(p)}$ be the vertex of $\mathcal{T}_n$ that holds the unique ball whose label contains $p$. Too see that at each step there is only one ball whose label contains $p$ almost surely, notice that the balls' labels form a partition of $[0,1]$ and recall that their endpoints are uniformly distributed over $[0,1]$. Thus, by definition of $T_n^{(p)}$ we have that $X_n^{(p)}$ must be a vertex of $T_n^{(p)}$, since its label contains the label of the ball that contains $p$, consequently it contains $p$. 

Now we show that the process $\{(T_n^{(p)},X_n^{(p)})\}_n$ is a Bernoulli instance of the TBRW with parameter $p$. We will argue that $T_n^{(p)}$ is actually a tree for all $n$ and that it is obtained from $T_{n-1}^{(p)}$ by adding a vertex to $X_{n-1}^{(p)}$ with probability $p$. Then, we will show that $X_n^{(p)}$ is a uniformly chosen neighbor of $X_{n-1}^{(p)}$ in $T_n^{(p)}$.


Towards that goal, firstly notice that $T_0^{(p)} = T$ and $X_0 = x$, since we labeled all of its vertices as $[0,1]$ and $x$ is the only vertex holding the ball with label $[0,1]$ (see Figure \ref{fig:supert0} for a reference with $v_3$ playing the role of $x$). Now we can argue by induction in the next paragraph.

Recall that in the process of labeling vertices, the vertices added to $\mathcal{T}_{n-1}$ in the $n$-th step are labeled as $[U_n,1]$ intersected by the union of disjoint intervals. Thus, if $U_n > p$, none of the new vertices are vertices of $T_n^{(p)}$, which means $T_n^{(p)} = T_{n-1}^{(p)}$. On the other hand, if $U_n < p$, we may gain new vertices whose label contains $p$. However, since there is only one ball whose label contains $p$, the only new vertex whose label will contain $p$ is the one attached to the position of the ball whose label contains $p$. Notice that the position of this ball is also a vertex of $T^{(p)}_{n-1}$ by construction. This shows $T_n^{(p)}$ is obtained from $(T_{n-1}^{(p)}, X_{n-1}^{(p)})$ by adding a vertex to $X_{n-1}^{(p)}$ with probability $p$.
%that if $\{(T^{(p)}_{j},X_j^{(p)})\}_{j=0}^{n-1}$ is distributed as the TBRW, so is $T^{(p)}_{n}$.

Now we need to show that $X^{(p)}_{n}$ has the right distribution, that is, it is a uniformly chosen neighbor of $X_{n-1}^{(p)}$ in $T_{n}^{(p)}$. We know that $X^{(p)}_{n}$ keeps track on the only ball the contains $p$. After sampling $U_n$, we still have only one ball whose label contains $p$. And notice that this ball jumps to a uniformly chosen vertex with label that contains the ball's label. Notice that all of the possible vertices for $X^{(p)}_{n}$ to jump are vertices of $T^{(p)}_{n}$ by definition. This shows that $X^{(p)}_{n}$ has the right distribution. \\

\noindent \underline{\it Part (b).} Assume w.l.o.g that $p<q$. We claim that the following inclusion of events holds
\begin{equation}\label{ineq:subset}
    \bigcap_{k=1}^n \{ U_k \notin (p,q)\} \subset \left \lbrace \left \lbrace\left( T_k^{(p)}, X_k^{(p)}\right)\right \rbrace_{k=0}^n = \left \lbrace\left( T_k^{(q)}, X_k^{(q)}\right)\right \rbrace_{k=0}^n \right \rbrace,
\end{equation}
which is enough to show part (b).

The proof follows by induction on $n$. Recall that at each step, if $[a,b]$ is the label of some ball in $\mathcal{T}_{k-1}$, then if $U_k \in [a,b]$, we replace this ball by two new ones with labels $[a,U_k]$ and $[U_k,b]$. Since we start with a single ball labeled $[0,1]$, the condition $U_1 \notin (p,q)$ implies that either $p,q$ are both in the ball labeled $[0,U_1]$ or in the ball labeled $[U_1,1]$. Regardless the cases, this implies that $X_1^{(p)} = X_1^{(q)}$. But notice that this also implies that $T_1^{(p)} = T_1^{(q)})$, since the new vertex added to $\mathcal{T}_1$ has label $[U_1,1]$, which either contains both $p$ and $q$ or none.

Thus, assume that \eqref{ineq:subset} holds for $n-1$, which additionally implies that there is a unique ball containing both $p$ and $q$. Given that, if $U_n \notin (p,q)$, we have that both $p$ and $q$ belong to the same ball in $\mathcal{T}_n$. Moreover, at step $n$, if $v$ is a vertex of $\mathcal{T}_{n-1}$ that receives a new vertex, this new vertex has label $[U_n,1] \cap (\text{union of the labels of balls on} v)$. Since $p$ and $q$ are both in the same ball, the condition $U_n \notin (p,q)$ implies again that the new vertex will be either visible to both $q$-TBRW and $p$-TBRW processes or to none of them. This shows \eqref{ineq:subset}, which shows part (b). \\



\noindent \underline{\it Part (c).} It is enough to observe that a vertex belongs to $T^{(p)}_n$ for some $n$ if its label contains $p$. Since vertice the new vertex attached to a given vertex $v$ is labeled as $[U_n,1] \cap (\text{union of the labels of balls on} v)$, the new vertex's label contains $p$ if and only if there is a ball  on $v$ whose label contains $p$ and $U_n < p$. Since at each step there is exactly one ball containing $p$, $V_n^{(p)} = |T| + \sum_{k=1}^n \mathds{1} \{U_k < p\}$, which is monotone increasly on $p$.



%Next, we move the only ball that contains $p$ uniformly among all the vertices whose label contains the label of this ball
%The fact that $T^{(p)}_n$ is a tree for $n\ge 1$ follows then by induction and construction. To see this, just notice that by construction there is only one ball containing $p$ at each step (due to continuous nature of $U$'s). And then, if $T_n^{(p)}$ is a tree, so is $T_{n+1}^{(p)}$ because the latter is obtained by possibly adding a new vertex to the position of the ball that contains $p$ in $\mathcal{T}_n$. 



%Now we need to show that the process $\{(T_n^{(p)},X_n^{(p)})\}_n$ is a Bernoulli instance of the TBRW with parameter $p$. We begin by observing that the probability of adding a new vertex to $(T_n^{(p)},X_n^{(p)})$ is $p$. Again, recall the process of labeling vertices. A new vertex of $\mathcal{T}_n$ is a vertex of $(T_n^{(p)},X_n^{(p)})$ if and only if its label contains $p$. As we observed before, if $U_n >p$, none of the new vertices added to $\mathcal{T}_{n-1}$ have label containing $p$. In the case $U_n < p$, we recall



%Notice that $T^{(p)}_1$ is either $T$ or $T$ together with a next vertex attached to $x$. The new vertex of $\mathcal{T}_1$ attached to $x$ is also a vertex of $T_1^{(p)}$ if and only if its label contains $p$. But notice that by construction this new vertex is labeled $[U_1,1]\cap [0,1]$. Thus, the new vertex is

%Next, we say that a vertex is {\it available} for a ball if the label on the ball (which is a interval) is contained in the vertex's label, which is also an interval. For instance, for the ball with label $[0,U_1]$ inside vertex $\ell$, the only vertex available is vertex $\ell -1$ whose label is $[0,1]$. On the other hand, for the ball with label $[U_1,1]$ we have two vertices available, $\ell -1$ and $\ell$. 

%Thus, for each ball, we select uniformly and independently an available vertex and move the ball to it. This new configuration is set as $\mathcal{X}_1$. That is, now $\mathcal{X}_1$ is a list of length $\ell +2$ together with two balls with labels $[0,U_1]$ and $[U_1,1]$.
\end{proof}



==> preliminaries.tex <==
\section{Preliminaries}\label{s:preliminaries}
Throughout the paper we will make use of some terminology that helps with the explanation as well as some shorthand in the notation to avoid clutter when there exists dependency on a high number of parameters.

\subsection{Notation and Terminology} Since we will measure the distance of the walker from the root, we will explore an analogy with genealogy trees. In this way, if $x\neq o$ is a vertex in $T_n$, for some $n$, we will refer to its only neighbor that is closer to the root as its father. And will denote this unique vertex by $f(x)$.

We will also need to {\it prone} trees at the father of given vertices. Thus, if $T$ is a rooted tree and $x \neq o$ one of its vertices, we will denote by $T(x)$ the subtree consisted of $x$ 




